Suzuki-Trotter Decompositions and other Methods for Quantum Time Evolution

(Suzuki-)Trotter decompositions, splitting methods, (Lie) product formulae... The most common numerical methods for the time evolution of quantum systems come with many names. And they are used practically everywhere with applications ranging from the solution of classical equations of motion and various Monte Carlo simulations to the real and imaginary time evolution on classical as well as quantum computers. Here we review the state of the art of said methods, focussing especially on the progress made over the last few years. We highlight recently discovered efficient time evolution algorithms and explain how best to use them in practice. A central part of this work is the estimation of error bounds that has improved greatly within the past decade. The relevance of time evolution methods for quantum computing is discussed with a focus on noisy hardware. Finally, a comprehensive overview of generalisations, related methods and alternatives to Trotterization is provided. This includes time-dependent Hamiltonian dynamics, processed methods, multi-product formulae, symplectic integrators, TDVP for tensor networks, quantum signal processing, Crouch-Grossman methods and more. The overall perspective in this work is that of a theoretical physicist. All mathematical proofs as well as some technical details are omitted for easier readability. Instead, this review serves as a hands-on guide and, of course, as a starting point for references that provide further details.

==> figures/Hahn-2410.03059v1.tex <==
\begin{tabular}{cc}
%	\multicolumn{1}{l}{\footnotesize(a)}
%	&
%	\multicolumn{1}{l}{\footnotesize(b)}
%	\\
	\begin{tikzpicture}[mark size={0.7}, scale=.89]
		\begin{axis}[
			xlabel={$t$},
			ylabel={error},
			tick label style={font=\footnotesize},
			x post scale=1.0,
			y post scale=0.8,
			legend cell align={left},
			legend pos=north west,
			ylabel near ticks,
			yticklabel pos=left,
			xmin=0,
			xmax=8,
			ymin=0,
			ymax=0.5,
			]
			\addplot[color=plotblue, thick, mark=*, only marks] table[x=t, y=error, col sep=comma] {paper-source/Hahn-2410.03059v1/XY_Norm_Time_Upper_Bound.csv};
			\addplot[color=plotorange, mark=*, only marks] table[x=t, y=error, col sep=comma] {paper-source/Hahn-2410.03059v1/XY_Norm_Time_Error.csv};
			\addplot[color=plotgreen, mark=*, only marks] table[x=t, y=error, col sep=comma] {paper-source/Hahn-2410.03059v1/XY_Norm_Time_Lower_Bound.csv};
			\addlegendimage{empty legend};
			\legend{
				\footnotesize Upper bound,
				\footnotesize Trotter error,
				\footnotesize Lower bound,
				\footnotesize {for $N_t=20$, $L=5$}
			};
		\end{axis}
	\end{tikzpicture}
	&
	\begin{tikzpicture}[mark size={1.5}, scale=.89]
		\begin{axis}[
			xmode=log,
			ymode=log,
			xlabel={$N_t$},
			ylabel={error},
			%label style={font=\footnotesize},
			tick label style={font=\footnotesize},
			x post scale=1,
			y post scale=0.8,
			legend pos=south west,
			legend columns=1,
			legend cell align={left},
			xmin=2, xmax=3000,
			]
			\addplot[color=1, mark=*, only marks] table[x=N, y=error, col sep=comma] {paper-source/Burgarth-2312.08044v2/Trotter_Error_2nd_order_groundstate_100.csv};
			\addplot[color=2, mark=*, only marks] table[x=N, y=error, col sep=comma] {paper-source/Burgarth-2312.08044v2/Trotter_Error_2nd_order_groundstate_200.csv};
			\addplot[color=3, mark=*, only marks] table[x=N, y=error, col sep=comma] {paper-source/Burgarth-2312.08044v2/Trotter_Error_2nd_order_groundstate_300.csv};
			\addplot[color=4, mark=*, only marks] table[x=N, y=error, col sep=comma] {paper-source/Burgarth-2312.08044v2/Trotter_Error_2nd_order_groundstate_400.csv};
			\addplot[color=5, mark=*, only marks] table[x=N, y=error, col sep=comma] {paper-source/Burgarth-2312.08044v2/Trotter_Error_2nd_order_groundstate_800.csv};
			\addplot[color=0, ultra thick, densely dashed, domain=2:3000]{0.15*x^(-2)};
			\addplot[color=6, ultra thick, domain=2:3000]{0.5*(2.04665*x^(-1/2) + 0.832107/x + 1.34365/x^(1/4))};
			\addplot[color=0, ultra thick, domain=2:3000]{0.31/x + 0.1/x^(1/2) + 0.1/x^(1/4)};
			\legend{
				\footnotesize $100$ modes,
				\footnotesize $200$ modes,
				\footnotesize $300$ modes,
				\footnotesize $400$ modes,
				\footnotesize $800$ modes,
				%\footnotesize $N_t^{-2}$,
				%\footnotesize analytic bound,
			};
		\end{axis}
		\node[color=6,rotate=-4] at (4,4.15) {\footnotesize upper bound $\ord(N_t^{-1/4})$};
		\node[color=0,rotate=-4] at (4,3.6) {\footnotesize scaling for $\infty$ modes};
		\node[color=0,rotate=-25] at (4.7,1.) {\footnotesize $\ord(N_t^{-2})$};
	\end{tikzpicture}
\end{tabular}

==> paper-source/Bosse-2403.08729v3/macros.tex <==
%\newcommand{\ttt}[1]{\texttt{#1}}
\newcommand{\icol}[1]{% inline column vector
  \left(\begin{matrix}#1\end{matrix}\right)%
}
\newcommand{\irow}[1]{% inline row vector
  \begin{matrix}(#1)\end{matrix}%
}
\newcommand{\absval}[1]{\left\lvert #1 \right\rvert} 

\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

\DeclareMathOperator{\diag}{diag}

\newcommand{\kk}{\bm{k}}
\newcommand{\RR}{\bm{R}}
\newcommand{\supp}{\text{supp}}
\newcommand{\dist}{\text{dist}}
% \newcommand{\THR}{THRIFT~}
% \newcommand{\FH}{Fermi-Hubbard~}
% \newcommand{\TFIM}{transverse field Ising~}
\newcommand{\THR}{THRIFT\xspace}
\newcommand{\apx}{apx\xspace}
\newcommand{\FH}{Fermi-Hubbard\xspace}
\newcommand{\TFIM}{transverse-field Ising model\xspace}
\newcommand{\HTFIM}{H_{\textnormal{TFIM}}}
\newcommand{\HFH}{H_{\textnormal{FH}}}
\newcommand{\HHeisenberg}{H_{\textnormal{Heisenberg}}}
% CD: Time ordering T macro
\newcommand{\T}{\mathcal{T}}
\newcommand{\hop}{t_{\mathrm{hop}}}

\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\diam}{diam}

% different norm macros
\newcommand\abs[1]{\lvert#1\rvert}
\newcommand\Abs[1]{\left|#1\right|}
\newcommand\norm[1]{\lVert#1\rVert}
\newcommand\Norm[1]{\left\|#1\right\|}
\newcommand\tracenorm[1]{\norm{#1}_{\text{tr}}}
\newcommand\Tracenorm[1]{\Norm{#1}_{\text{tr}}}
\newcommand\onenorm[1]{\norm{#1}_1}
\newcommand\Onenorm[1]{\Norm{#1}_1}
\newcommand\twonorm[1]{\norm{#1}_2}
\newcommand\Twonorm[1]{\Norm{#1}_2}

\newcommand{\am}[1]{{\color{magenta} AM: #1}}
\newcommand{\fmg}[1]{{\color{blue} FMG: #1}}
\newcommand{\rs}[1]{{\color{blue} RS: #1}}
\newcommand{\old}[1]{{\color{gray} OLD VERSION: #1}}
\newcommand{\jlb}[1]{{\color{green} JLB: #1}} 
\newcommand{\amc}[1]{{\color{orange} AMC: #1}}
\newcommand{\cd}[1]{{\color{red} CD: #1}}


==> paper-source/Bosse-2403.08729v3/preamble.tex <==
%%%%%%%%%%%%%%%
%% Keep useful packages here that will be wanted in most projects 
%% Add less common packages on a per-project basis
%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%
%% Defaults
%%%%%%%%%%%%%%%
\usepackage[a4paper, total={7in, 9in}]{geometry}
%\usepackage[utf8]{inputenc}
\usepackage{tikz}
%\usepackage{background}
\usepackage{caption}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage[normalem]{ulem}

\usepackage{longtable}
\usepackage{comment}

\usepackage[
    backend=bibtex,
    natbib = true,
    style = phys,
    isbn = false,
    hyperref = true,
    sorting = none,
    giveninits = true,
    maxbibnames = 9,
    biblabel = brackets,
    eprint = true
]{biblatex}

\bibliography{references}


%%%%%%%%%%%%%%%
%% Maths
%%%%%%%%%%%%%%%
\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{braket}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Figures, in particular PGF figures
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{tikz}
\usepackage{pgfplots}
% stuff to include the figures from elsewhere
\graphicspath{{figures/}{.}}
\makeatletter
\def\input@path{{figures/}{.}}
%or: \def\input@path{{/path/to/folder/}{/path/to/other/folder/}}
\makeatother

% whack shit to get the pngs in the pgf to be included correctly
\pgfplotsset{compat=1.16}
\providecommand\inputpgf[2]{{
\let\pgfimageWithoutPath\pgfimage
\renewcommand{\pgfimage}[2][]{\pgfimageWithoutPath[##1]{#1/##2}}
\input{#1/#2}
}}

%%%%%%%%%%%%%%%
%% Miscellaneous useful stuff
%%%%%%%%%%%%%%%
\usepackage{listings}
\usepackage[ruled,vlined]{algorithm2e}
\usepackage{amssymb}
\usepackage[ampersand]{easylist}
\usepackage{enumitem}
\usepackage{hyperref}
\hypersetup{
  colorlinks = true, %Colours links instead of ugly boxes
  linkcolor={blue!50!black}, %Colour of internal links
  citecolor=red, %{red!50!black}, %Colour of citations
  urlcolor=blue, %Colour for external hyperlinks
  linktoc=page,
}
\usepackage[capitalise, nameinlink]{cleveref}
\usepackage[
  style=long,
  nolist, 
  nonumberlist,
  nopostdot,
  acronym,
  toc=true, 
]{glossaries}
\usepackage{bm}
\usepackage{booktabs}
\usepackage{multirow}
\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\usepackage{array}
\usepackage[british]{babel}


\newtheorem{theorem}{Theorem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}

\newcommand{\SubItem}[1]{
    {\setlength\itemindent{15pt} \item[-] #1}
}

\usepackage{makecell}

\usepackage{xspace}

% fix spacing of \left and \right delimeters
\let\originalleft\left
\let\originalright\right
\renewcommand{\left}{\mathopen{}\mathclose\bgroup\originalleft}
\renewcommand{\right}{\aftergroup\egroup\originalright}
